IsoAlign: Isoform-Aware DNA-Protein Alignment via Joint-Embedding Predictive Architectures

Genomic foundation models (GFMs) have emerged as a powerful paradigm for learning DNA sequence representations, yet existing self-supervised pretraining strategies overlook alternative splicing and underperform compared to specialized models. To address this gap, we introduce IsoAlign, a multimodal framework that grounds genomic pretraining in isoform-aware DNA-protein alignment to learn biologically meaningful representations. IsoAlign aligns transcripts to their corresponding protein isoforms, capturing both coding sequences and broader regulatory contexts, using two Joint-Embedding Predictive Architectures (JEPA): DNA-Protein JEPA (DP-JEPA), which predicts protein representations from DNA using contrastive alignment, and Isoform-Masked JEPA (IM-JEPA), which models relationships among alternative isoforms of the same gene through masked protein prediction. We evaluate the learned DNA representations of these architectures across a multi-metric evaluation suite spanning tasks, including the prediction of pathogenicity, fitness, gene expression, and TF binding. Our results demonstrate that isoform-aware cross-modal alignment using JEPA significantly improves functional representations and downstream performance, establishing a promising direction for GFM pretraining.

==> sections/5_objectives.tex <==
    
\section{Pretraining Objectives}
\label{sec:pretraining_obj}

\textcolor{red}{To isolate the performance gains of our JEPA objectives from the underlying dual-encoder architecture and increased parameter count, we implement several architecture-matched controls. These controls utilize the exact same DNA encoder, frozen protein encoder, and projection heads, but replace the JEPA objective with masked language modelling or contrastive losses:}

  \paragraph{Masked Language Modeling (MLM).}
  We implement four MLM configurations with a 15\% masking rate. Cross-modal conditioning utilizes either \textbf{sequence-level} (global pooling) or \textbf{token-level} (position-specific) multi-head
  cross-attention (8 heads), with linear projections to align hidden dimensions between modalities.
  \begin{enumerate}                                         
      \item \textbf{Standard Joint:} Independent MLM with combined loss:  $\mathcal{L}_{\mathrm{Joint}} = \lambda_D \mathcal{L}_{\mathrm{MLM}}^D + \lambda_P \mathcal{L}_{\mathrm{MLM}}^P$.
 
      \item \textbf{P$\rightarrow$D:} Unmasked protein predicts masked DNA:
      $\hat{\mathbf{H}}_D \!=\! \mathrm{LN}(\mathrm{Attn}(\mathbf{H}_D, \mathbf{W}_P\mathbf{H}_P) \!+\! \mathbf{H}_D)$.
      \item \textbf{D$\rightarrow$P:} Unmasked DNA predicts masked protein:
      $\hat{\mathbf{H}}_P \!=\! \mathrm{LN}(\mathrm{Attn}(\mathbf{H}_P, \mathbf{W}_D\mathbf{H}_D) \!+\! \mathbf{H}_P)$.
      \item \textbf{Bidirectional:} Both modalities are masked; combines (2) and (3) for mutually enhanced reconstruction.
  \end{enumerate}
  
\paragraph{Contrastive Learning.}
We align DNA-protein embeddings using three loss variants, governed by a biological correctness matrix $\mathbf{C} \in \{0, 1\}^{N \times N}$. All variants utilize a 8,192-entry momentum memory bank ($m=0.999$) \citep{he2020moco}.

\begin{itemize}
    \item \textbf{InfoNCE:} Maximizes matched-pair similarity using learnable temperature $\tau$ (init 0.5).
    % Maximizes agreement between matched pairs using learnable temperature $\tau$ (init 0.5).
    \item \textbf{DCL:} Decoupled loss~\citep{yeh2022decoupled} separating positive and negative terms for independent weighting: $\mathcal{L}_{\text{DCL}} = \lambda_{\text{pos}}(-\bar{s}_{\text{pos}}) + \lambda_{\text{neg}}\log\sum\exp(s_{\text{neg}})$.
    %  \item \textbf{DCL:} Decoupled loss separating positive and negative terms with cross-view and same-view negatives: $\mathcal{L}_{\text{DCL}} = \lambda_{\text{pos}}(-\bar{s}_{\text{pos}}) +              
    %  \lambda_{\text{neg}}(\log\sum\exp(s_{\text{cross}}) + \log\sum\exp(s_{\text{same}}))$   
    \item \textbf{CLIP:} Symmetric bidirectional NCE with low initial temperature ($\tau_0=0.1$, learnable) for sharp distribution alignment \cite{radford2021learning}.
\end{itemize}

  \textcolor{red}{should highlight that isoform masked jepa requires genes with mulitple isoforms and highlight that as the major contribution there}
  
\subsection{DNA-Protein JEPA}                                                                  
\paragraph{Architecture.} We introduce DNA-Protein Joint-Embedding Predictive Architecture (DP-JEPA), a cross-modal self-supervised framework that learns to predict protein representations from DNA sequences in a shared latent space, outlined in Figure \ref{fig:jepa}a. It consists of: (1) a trainable DNA encoder $f_\theta$, (2) a protein encoder $g_\phi$ (frozen by default), and (3) a TransformerPredictor $h_\psi$ that predicts protein embeddings from DNA representations.

The TransformerPredictor is a stack of transformer encoder layers (default: 4 layers, 8 heads) that processes the full sequence of DNA hidden states with attention masking, then mean-pools across valid positions:
  \begin{equation}
      \hat{\mathbf{z}}_y = \pi_{\text{pred}}\bigl(\mathrm{LN}(\mathrm{MeanPool}(h_\psi(\mathbf{H}_x, \mathbf{m}_x)))\bigr),
  \end{equation}
where $\mathbf{m}_x$ is the attention mask excluding padding tokens.

The target protein embedding applies stop-gradient to the encoder output while keeping the projection trainable:
  \begin{equation}
      \mathbf{z}_y = \pi_y\bigl(\mathrm{sg}(\mathrm{pool}(g_\phi(\mathbf{y})))\bigr).
  \end{equation}

  Both $\pi_{\text{pred}}$ and $\pi_y$ are multi-layer projection heads mapping to a shared embedding space.

\paragraph{Training Objective.} DP-JEPA employs contrastive alignment in the shared projection space. For a batch of genes, each potentially having multiple protein isoforms, we compute the loss per isoform slot and average:
  \begin{equation}
      \mathcal{L}_{\text{DP-JEPA}} = \frac{1}{|\mathcal{V}|}\sum_{j \in \mathcal{V}}
      \mathcal{L}_{\text{contrast}}(\hat{\mathbf{Z}}_y, \mathbf{Z}_{y_j}; \tau),
  \end{equation} where $\mathcal{V}$ denotes valid isoform slots (non-padded entries with $\geq 2$ samples for contrastive discrimination). The target projection $\pi_y$ is frozen under stop-gradient to provide stable targets.


\paragraph{Isoform-Masked JEPA.} While DP-JEPA aligns each transcript-protein isoform pair through cross-modal prediction, it does not explicitly model relationships among alternative isoforms of the same gene. To incorporate this intra-gene structure, we introduce Isoform-Masked JEPA (IM-JEPA), which jointly processes multiple transcript--isoform pairs and predicts masked protein isoforms from their DNA anchors and the remaining visible isoform context. Specifically, for genes with multiple transcript-isoform pairs
    $\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^N$, we extend DP-JEPA with object-level masking
    inspired by Causal-JEPA~\citep{nam2026causal}, outlined in Figure \ref{fig:jepa}b. Approximately 50\% of isoforms are randomly
    masked per sample while all DNA anchors remain visible, ensuring at least one isoform
    stays visible for context. The predictor operates on \emph{pooled} encoder representations
    and employs three types of learnable embeddings: (1) modality embeddings distinguishing
    DNA from protein isoforms, (2) slot embeddings indexing each pair, and
    (3) a learnable mask token $\mathbf{m}$. For masked isoforms, we inject \emph{identity
    queries} derived from their DNA anchors via a learned projection $\rho$:
    \begin{equation}
        \mathbf{s}_i^{\text{iso}} = \begin{cases}
            \pi_{\text{iso}}(\mathbf{z}_{\mathbf{y}_i}) + \mathbf{e}_{\text{iso}} + \mathbf{e}_i & \text{if visible} \\
            \mathbf{m} + \rho(\pi_{\text{dna}}(\mathbf{z}_{\mathbf{x}_i})) + \mathbf{e}_{\text{iso}} + \mathbf{e}_i & \text{if masked}
        \end{cases},
    \end{equation}
    where $\mathbf{z}_{\mathbf{x}_i} = \text{pool}(f_\theta(\mathbf{x}_i))$ and
    $\mathbf{z}_{\mathbf{y}_i} = \text{pool}(g_\phi(\mathbf{y}_i))$ are pooled encoder outputs,
    and $\pi_{\text{dna}}$, $\pi_{\text{iso}}$ are input projections with layer normalization.

    The full input sequence concatenates all DNA representations with isoform
    representations, processed by a bidirectional Transformer encoder:
    \begin{equation}
        \hat{\mathbf{Z}} = h_\psi\bigl([\pi_{\text{dna}}(\mathbf{z}_{\mathbf{x}}^{(1:N)}) + \mathbf{e}_{\text{dna}} + \mathbf{e}_{\text{slot}};\; \mathbf{s}^{(1:N)}]\bigr).
    \end{equation}

    The loss is computed on masked and valid (non-padded) positions using $\ell_2$-normalized embeddings:
    \begin{equation}
        \mathcal{L}_{\text{IM-JEPA}} = \frac{1}{|\mathcal{M} \cap \mathcal{V}|} \sum_{i \in \mathcal{M} \cap \mathcal{V}} \bigl\|\bar{\hat{\mathbf{z}}}_i - \bar{\mathbf{z}}_i\bigr\|_2^2 +
  \lambda_{\text{reg}}
     \mathcal{L}_{\text{SIGReg}},
    \end{equation}
    where $\bar{\mathbf{z}} = \mathbf{z} / \|\mathbf{z}\|_2$, $\mathcal{M}$ denotes masked positions,
    $\mathcal{V}$ denotes valid (non-padded) pairs, and $\mathcal{L}_{\text{SIGReg}}$ enforces
    $\mathcal{N}(0, \mathbf{I})$ statistics on predictions to prevent representational collapse.

\paragraph{SIGReg Anti-Collapse Regularization.} To prevent representational collapse, we employ SIGReg \citep{balestriero2025lejepa}, which encourages predictions to follow an isotropic Gaussian $\mathcal{N}(0, \mathbf{I})$ via characteristic function matching. Predictions are projected onto $K$ random unit vectors $\{\mathbf{p}_k\}_{k=1}^{K}$ (resampled each iteration) and compared to the Gaussian characteristic function $\varphi(t) = e^{-t^2/2}$:                     
\begin{equation}
      \mathcal{L}_{\text{SIGReg}} = \frac{1}{K}\sum_{k=1}^{K} \int_0^{t_{\max}} w(t) \left[                                                                    
      \bigl(\bar{c}_k(t) - e^{-t^2/2}\bigr)^2 + \bar{s}_k(t)^2 \right] dt,                                    
\end{equation}
where $\bar{c}_k(t) = \mathbb{E}[\cos(t \cdot \mathbf{p}_k^\top \hat{\mathbf{z}})]$ and $\bar{s}_k(t) = \mathbb{E}[\sin(t \cdot \mathbf{p}_k^\top \hat{\mathbf{z}})]$ are empirical characteristic function components, and $w(t) \propto e^{-t^2/2}$ weights errors by target magnitude. We use $K{=}1024$ projections with trapezoidal integration over $t \in [0, 3]$.  

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/architecture_overview.pdf}
%     \caption{}
%     \label{fig:Arch_overview}
% \end{figure}



\begin{figure}[t]
    \centering

    % --- First subfigure ---
    \begin{subfigure}{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/DP-JEPA.png}
        \caption{\textbf{DP-JEPA (DNA-Protein Joint-Embedding Predictive Architecture):} A dual-encoder framework where DNA sequences are processed by a trainable DNA encoder (e.g., NTv2) and projected through a Transformer predictor to align with protein representations from a frozen protein encoder (e.g., ESM2). The model learns cross-modal alignment via contrastive loss in a shared latent space.}
        % , with stop-gradient applied to protein targets.}
        \label{fig:sub1}
    \end{subfigure}

    \vspace{0.2cm}

    % --- Second subfigure ---
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/IM-JEPA.png}
        \caption{\textbf{IM-JEPA (Isoform-Masked JEPA):} An extension of DP-JEPA that jointly models multiple transcript-isoform pairs from the same genes. DNA sequences for all isoforms are encoded and pooled, while protein isoforms are randomly masked ($\sim$50\%). The Transformer Predictor uses DNA anchors as identity queries to predict masked protein embeddings, with L2-normalized MSE loss computed only on masked positions and SIGReg regularization to prevent collapse.}
        \label{fig:sub2}
    \end{subfigure}

    \caption{\textbf{\textsc{IsoAlign} JEPA Architectures}}
    \label{fig:jepa}
\end{figure}


  

==> tables/imjepa_ablation.tex <==
\begin{table}[[htbp]]
\centering
\caption{Isoform Masked JEPA ablation study across zero-shot variant effect prediction (VEP) and deep mutational scanning (DMS) benchmarks.}
\label{tab:jepa-ablation}
\begin{tabular}{lllcc}
    \toprule
    Mask & Level & Species & VEP & DMS \\
    \midrule
    \multicolumn{5}{l}{\textit{Mask Ratio}} \\
    0.25 & 4 & Human & - & - \\
    0.50 & 4 & Human & - & - \\
    0.75 & 4 & Human & - & - \\
    Dense & 4 & Human & - & - \\
    \midrule
    \multicolumn{5}{l}{\textit{Supervision Level}} \\
    0.50 & 1 & Human & - & - \\
    0.50 & 4 & Human & - & - \\
    0.50 & 8 & Human & - & - \\
    \midrule
    \multicolumn{5}{l}{\textit{Species Filtering}} \\
    0.50 & 4 & MSigDB & - & - \\
    0.50 & 4 & Human & - & - \\
    \midrule
    \multicolumn{5}{l}{\textit{Loss Type}} \\
    0.50 & 4 & Human & - & - \\
    EMA & 4 & Human & - & - \\
    Dense & 4 & Human & - & - \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/tfiso.tex <==
  \begin{table}[htbp]                              
      \centering                                   
      \caption{Zero-shot evaluation of isoform-specific TF-DNA binding properties. The best model per pretraining objective is reported.}                                    
      \label{tab:tfiso_results}
      \small                                       
      \begin{tabular}{llccc}                       
      \toprule                                     
      \textbf{Objective} & \textbf{DNA FM} & \textbf{PDI (AUC)} & \textbf{PBM ($\rho$)} & \textbf{Rank} $\downarrow$ \\
      \midrule
      LucaOne~\citep{he2025generalized} & -- & 0.551 $\pm$ 0.10 & \textbf{0.912} & 3.0 \\
      \midrule
      IsoAlign DP-JEPA & NTv2 & \underline{0.615 $\pm$ 0.10} & 0.900 & \textbf{2.5} \\
      IsoAlign IM-JEPA & AG & 0.612 $\pm$ 0.10 & \underline{0.911} & \textbf{2.5} \\
      Contrastive & NTv2 & \textbf{0.618 $\pm$ 0.09} & 0.890 & 3.0 \\
      MLM & NTv2 & 0.608 $\pm$ 0.12 & 0.891 & 4.0 \\
      \bottomrule
      \end{tabular}
  \end{table}

==> tables/zero-shot-dms.tex <==
  \begin{table}[htbp]                           
    \centering
    \caption{DMS Variant Effect Prediction (Spearman $\rho$). Best results \textbf{bolded}, second best \underline{underlined} per column.}            
    \label{tab:dms_results}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llcccccc}
    \toprule
    \textbf{Category} & \textbf{Model} & \textbf{Garvie} & \textbf{Giacomelli} & \textbf{Kotler} & \textbf{Silverstein} & \textbf{Sun} & \textbf{Mean} \\
    \midrule
    \multicolumn{8}{l}{\textit{DNA Foundation Models}} \\
    & NTv2-500M &  &  &  &  &  &  \\ 
    & Evo2-7B & 0.26 & 0.30 & 0.30 & 0.14 & 0.31 & 0.26 \\
    & NTv3-650M & 0.26 & 0.24 & 0.37 & 0.10 & 0.38 & 0.27 \\
    & AIDO & 0.05 & 0.11 & 0.24 & 0.02 & 0.14 & 0.11 \\
    & HyenaDNA & 0.03 & 0.03 & 0.22 & 0.03 & 0.04 & 0.07 \\
    & Caduceus-PS & 0.06 & 0.08 & 0.14 & 0.06 & 0.02 & 0.07 \\
    & LucaOne & 0.08 & 0.16 & 0.11 & 0.04 & 0.06 & 0.09 \\
    & OmniDNA 300M & 0.01 & 0.02 & 0.14 & 0.03 & 0.06 & 0.05 \\
    & DNABERT-2 & 0.01 & 0.01 & 0.14 & 0.01 & 0.04 & 0.04 \\
    \midrule
    \multicolumn{8}{l}{\textit{Protein Foundation Models}} \\
    & ESM-2 & 0.48 & 0.80 & \underline{0.69} & 0.15 & 0.54 & 0.53 \\
    & ESM-C 600M & \textbf{0.51} & \underline{0.83} & \underline{0.69} & 0.15 & \underline{0.55} & \textbf{0.55} \\
    & ESM-C 300M & \underline{0.50} & 0.82 & 0.68 & 0.12 & \underline{0.55} & 0.53 \\
    & ESM-1b & 0.46 & 0.82 & 0.61 & 0.11 & 0.51 & 0.50 \\
    & ESM-1v & 0.48 & 0.82 & 0.61 & 0.12 & 0.54 & 0.51 \\
    & ProtT5 & 0.49 & 0.80 & 0.64 & 0.12 & 0.54 & 0.52 \\
    \midrule
    \multicolumn{8}{l}{\textit{IsoAlign -- MLM}} \\
    & Standard Joint & 0.40 & 0.82 & 0.47 & 0.12 & 0.48 & 0.46 \\
    & Prot$\rightarrow$DNA (seq) & 0.41 & 0.80 & 0.50 & 0.12 & 0.48 & 0.46 \\
    & Prot$\rightarrow$DNA (token) & 0.41 & 0.81 & 0.50 & 0.12 & 0.47 & 0.46 \\
    & DNA$\rightarrow$Prot & 0.36 & 0.75 & 0.55 & 0.12 & 0.43 & 0.44 \\
    & Bidirectional & 0.39 & 0.78 & 0.60 & 0.11 & 0.46 & 0.47 \\
    \midrule
    \multicolumn{8}{l}{\textit{IsoAlign -- Contrastive}} \\
    & InfoNCE & 0.40 & 0.81 & 0.57 & 0.14 & 0.47 & 0.48 \\
    & DCL & 0.41 & 0.82 & \underline{0.69} & 0.22 & 0.54 & \underline{0.54} \\
    & CLIP & 0.41 & \underline{0.83} & \textbf{0.70} & \underline{0.23} & \underline{0.55} & \underline{0.54} \\
    \midrule
    \multicolumn{8}{l}{\textit{IsoAlign -- DP-JEPA}} \\
    & InfoNCE & 0.42 & \underline{0.83} & 0.61 & 0.13 & 0.48 & 0.49 \\
    & DCL & 0.39 & \textbf{0.84} & \textbf{0.70} & \textbf{0.24} & 0.53 & \underline{0.54} \\
    & CLIP & 0.40 & \textbf{0.84} & \underline{0.69} & \underline{0.23} & \textbf{0.56} & \underline{0.54} \\
    \midrule
    \multicolumn{8}{l}{\textit{IsoAlign -- Isoform-Masked JEPA}} \\
    & IM-JEPA & 0.40 & 0.79 & 0.53 & 0.13 & 0.47 & 0.47 \\
    \bottomrule
    \end{tabular}%
    }
  \end{table}

==> tables/zero-shot_with_final_splicing.tex <==
\begin{table*}[htbp]                           
    \centering
    \caption{Zero-shot variant effect prediction evaluation across metrics}
    \label{tab:zero-shot-eval}            
 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccccc}                                                         
        \toprule
        & & \multicolumn{4}{c}{ClinVar missense}
        & \multicolumn{4}{c}{ClinVar Splicing}
        & \multicolumn{4}{c}{MFASS} \\

        \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14}

        Model & Params
        & Cos & L2 & CLS & Mul
        & Cos & L2 & CLS & Mul
        & Cos & L2 & CLS & Mul \\

        \midrule

        \multicolumn{14}{l}{\textbf{Baselines}} \\
    Alphagenome & 450M & 0.46 & 0.47 & 0.52 & 0.74 & \underline{0.61} & 0.57 & \underline{0.67} & 0.46 & 0.29 & \underline{0.31} & \textbf{0.45} & \textbf{0.60} \\
    NT & 500M & 0.40 & 0.54 & 0.52 & 0.70 & 0.32 & 0.73 & 0.53 & 0.50 & 0.04 & 0.04 & 0.05 & 0.10 \\
    DNABERT-2 & 117M & 0.44 & 0.45 & 0.47 & 0.67 & 0.14 & 0.15 & 0.19 & 0.25 & 0.04 & 0.04 & 0.05 & 0.07 \\
    HyenaDNA & 1.6M & 0.48 & 0.49 & 0.49 & 0.60 & 0.17 & 0.18 & 0.25 & 0.22 & 0.04 & 0.04 & 0.05 & 0.07 \\
    Caduceus-PH & 7.7M & 0.46 & 0.48 & 0.48 & 0.64 & 0.20 & 0.18 & 0.20 & 0.24 & 0.04 & 0.04 & 0.05 & 0.08 \\
    Caduceus-PS & 7.7M & 0.46 & 0.47 & 0.50 & 0.67 & 0.20 & 0.45 & 0.43 & 0.46 & 0.04 & 0.08 & 0.15 & 0.18 \\
    LucaOne & 1.8B & 0.46 & 0.47 & 0.46 & 0.62 & 0.15 & 0.16 & 0.18 & 0.23 & 0.05 & 0.06 & 0.11 & 0.27 \\
    LucaOne-gene & 1.8B & 0.47 & 0.46 & 0.47 & 0.62 & 0.15 & 0.17 & 0.19 & 0.24 & 0.05 & 0.06 & 0.10 & 0.28 \\
    Orthrus-4track & 10M & 0.47 & 0.46 & 0.44 & 0.59 & 0.18 & 0.16 & 0.14 & 0.22 & 0.04 & 0.04 & 0.04 & 0.07 \\
    Omni-DNA-116M & 116M & 0.45 & 0.44 & 0.54 & 0.71 & 0.15 & 0.15 & 0.56 & 0.28 & 0.04 & 0.04 & 0.11 & 0.16 \\
    Omni-DNA-300M & 300M & 0.45 & 0.44 & 0.51 & 0.72 & 0.15 & 0.14 & 0.50 & 0.29 & 0.04 & 0.04 & 0.15 & 0.18 \\
    AIDO.DNA-300M & 300M & 0.59 & \underline{0.62} & 0.55 & 0.74 & 0.52 & 0.58 & 0.54 & \textbf{0.58} & 0.05 & 0.09 & 0.14 & 0.22 \\
    NTv3-650M & 650M & 0.56 & 0.50 & 0.49 & \underline{0.76} & 0.35 & 0.57 & 0.36 & 0.41 & 0.04 & 0.07 & 0.13 & 0.30 \\
    Evo2-1B-base & 1B & 0.56 & 0.77 & 0.57 & 0.79 & 0.38 & 0.85 & 0.60 & 0.51 & 0.05 & 0.16 & 0.20 & 0.41 \\
    Evo2-7B-base & 7B & \textbf{0.70} & \textbf{0.79} & \textbf{0.79} & \textbf{0.81} & 0.57 & \textbf{0.88} & \textbf{0.72} & \underline{0.57} & 0.05 & 0.09 & 0.21 & 0.46 \\

        \midrule

    \multicolumn{14}{l}{\textbf{Ours [NT-ESM2]}} \\
    DPJEPA (CLIP) & 520M & 0.55 & 0.61 & 0.55 & 0.75 & \textbf{0.63} & 0.67 & 0.49 & 0.52 & 0.08 & 0.17 & 0.21 & 0.26 \\
    IMJEPA & 520M & 0.46 & 0.59 & 0.56 & 0.71 & 0.35 & \underline{0.74} & 0.60 & 0.54 & 0.04 & 0.05 & 0.08 & 0.12 \\
    Bidirectional TCA & 1.15B & 0.57 & 0.60 & \underline{0.58} & 0.73 & 0.50 & 0.61 & 0.64 & 0.55 & 0.04 & 0.04 & 0.05 & 0.10 \\
    DPJEPA (InfoNCE) & 520M & 0.58 & 0.60 & 0.56 & 0.73 & 0.58 & 0.55 & 0.60 & 0.32 & 0.07 & 0.12 & 0.18 & 0.22 \\
    MLM & 1.15B & 0.41 & 0.55 & 0.55 & 0.70 & 0.27 & 0.73 & 0.60 & 0.47 & 0.04 & 0.04 & 0.07 & 0.10 \\
    Conditioned MLM & 1.15B & 0.41 & 0.55 & 0.53 & 0.71 & 0.27 & 0.73 & 0.54 & 0.48 & 0.04 & 0.04 & 0.06 & 0.10 \\
    DPJEPA (DCL) & 520M & 0.58 & \underline{0.62} & 0.55 & 0.73 & 0.39 & 0.47 & 0.50 & 0.32 & 0.05 & 0.06 & 0.11 & 0.15 \\
    Contrastive (CLIP) & 1.15B & 0.43 & 0.60 & 0.50 & 0.72 & 0.40 & 0.70 & 0.48 & \textbf{0.58} & 0.04 & 0.07 & 0.08 & 0.12 \\
    Contrastive (InfoNCE) & 1.15B & 0.45 & 0.60 & 0.51 & 0.72 & 0.39 & 0.69 & 0.47 & \textbf{0.58} & 0.05 & 0.09 & 0.08 & 0.14 \\
    Cross-Modal & 1.15B & \underline{0.61} & 0.60 & 0.50 & 0.72 & 0.52 & 0.48 & 0.43 & 0.47 & 0.04 & 0.05 & 0.07 & 0.10 \\
    Contrastive (DCL) & 1.15B & 0.46 & 0.59 & 0.50 & 0.75 & 0.47 & 0.64 & 0.40 & 0.64 & 0.04 & 0.05 & 0.06 & 0.11 \\

    \multicolumn{14}{l}{\textbf{[AlphaGenome-ESM2]}} \\
    DPJEPA (CLIP) & 470M & 0.47 & 0.50 & 0.53 & 0.73 & \textbf{0.63} & 0.60 & 0.66 & 0.44 & \textbf{0.36} & \underline{0.31} & \underline{0.44} & \underline{0.59} \\
    IMJEPA & 470M & 0.47 & 0.46 & 0.51 & 0.73 & 0.33 & 0.30 & 0.61 & 0.33 & 0.06 & 0.09 & 0.29 & 0.43 \\

    \multicolumn{14}{l}{\textbf{[AlphaGenome-E1]}} \\
    DPJEPA (CLIP) & 470M & 0.47 & 0.49 & 0.52 & 0.74 & \textbf{0.63} & 0.60 & \underline{0.67} & 0.48 & \underline{0.32} & \textbf{0.34} & 0.43 & \underline{0.59} \\
    IMJEPA & 470M & 0.46 & 0.46 & 0.49 & 0.72 & 0.28 & 0.26 & 0.56 & 0.31 & 0.08 & 0.15 & 0.32 & 0.44 \\

        \bottomrule
    \end{tabular}
    }
    \end{table*}


==> tables/zero-shot_with_final_splicing_LOCO.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Zero-shot variant effect prediction evaluation across metrics}
  \label{tab:zero-shot-eval}

  \resizebox{\textwidth}{!}{
  \begin{tabular}{lccccccccccccc}
      \toprule
      & & \multicolumn{4}{c}{ClinVar missense}
      & \multicolumn{4}{c}{ClinVar Splicing}
      & \multicolumn{4}{c}{MFASS} \\

      \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14}

      Model & Params
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul \\

      \midrule

      \multicolumn{14}{l}{\textbf{Baselines}} \\
  Alphagenome & 450M & 0.46 & 0.47 & 0.51 & 0.58 & \underline{0.61} & 0.57 & \underline{0.63} & 0.30 & 0.29 & \underline{0.31} & \underline{0.32} & \textbf{0.23} \\
  NT & 500M & 0.40 & 0.54 & 0.52 & 0.66 & 0.32 & 0.73 & 0.52 & 0.42 & 0.04 & 0.04 & 0.05 & 0.04 \\
  DNABERT-2 & 117M & 0.44 & 0.45 & 0.46 & 0.58 & 0.14 & 0.15 & 0.18 & 0.18 & 0.04 & 0.04 & 0.05 & 0.04 \\
  HyenaDNA & 1.6M & 0.48 & 0.49 & 0.49 & 0.54 & 0.17 & 0.18 & 0.25 & 0.18 & 0.04 & 0.04 & 0.05 & 0.04 \\
  Caduceus-PH & 7.7M & 0.46 & 0.48 & 0.48 & 0.58 & 0.20 & 0.18 & 0.19 & 0.19 & 0.04 & 0.04 & 0.05 & 0.05 \\
  Caduceus-PS & 7.7M & 0.46 & 0.47 & 0.49 & 0.61 & 0.20 & 0.45 & 0.42 & 0.42 & 0.04 & 0.08 & 0.13 & 0.10 \\
  LucaOne & 1.8B & 0.46 & 0.47 & 0.46 & 0.50 & 0.15 & 0.16 & 0.18 & 0.17 & 0.05 & 0.06 & 0.09 & 0.07 \\
  LucaOne-gene & 1.8B & 0.47 & 0.46 & 0.47 & 0.51 & 0.15 & 0.17 & 0.18 & 0.17 & 0.05 & 0.06 & 0.08 & 0.06 \\
  Orthrus-4track & 10M & 0.47 & 0.46 & 0.46 & 0.48 & 0.18 & 0.16 & 0.14 & 0.16 & 0.04 & 0.04 & 0.04 & 0.04 \\
  Omni-DNA-116M & 116M & 0.45 & 0.44 & 0.54 & 0.62 & 0.15 & 0.15 & 0.55 & 0.21 & 0.04 & 0.04 & 0.10 & 0.06 \\
  Omni-DNA-300M & 300M & 0.45 & 0.44 & 0.50 & 0.63 & 0.15 & 0.14 & 0.49 & 0.21 & 0.04 & 0.04 & 0.13 & 0.06 \\
  AIDO.DNA-300M & 300M & 0.59 & \underline{0.62} & 0.54 & 0.66 & 0.52 & 0.58 & 0.52 & \underline{0.52} & 0.05 & 0.09 & 0.12 & 0.07 \\
  NTv3-650M & 650M & 0.56 & 0.50 & 0.48 & 0.66 & 0.35 & 0.57 & 0.34 & 0.28 & 0.04 & 0.07 & 0.08 & 0.07 \\
  Evo2-1B-base & 1B & 0.56 & 0.77 & 0.57 & 0.67 & 0.38 & 0.85 & 0.59 & 0.35 & 0.05 & 0.16 & 0.16 & 0.10 \\
  Evo2-7B-base & 7B & \textbf{0.70} & \textbf{0.79} & \textbf{0.79} & \underline{0.67} & 0.57 & \textbf{0.88} & \textbf{0.72} & 0.36 & 0.05 & 0.09 & 0.13 & 0.13 \\

      \midrule


  \multicolumn{14}{l}{\textbf{Ours [NT-ESM2]}} \\
  DPJEPA (CLIP) & 520M & 0.55 & 0.61 & 0.54 & \underline{0.67} & \textbf{0.63} & 0.67 & 0.47 & 0.46 & 0.08 & 0.17 & 0.18 & 0.08 \\
  DPJEPA (DCL) & 520M & 0.58 & \underline{0.62} & 0.55 & 0.65 & 0.39 & 0.47 & 0.49 & 0.24 & 0.05 & 0.06 & 0.10 & 0.06 \\
  DPJEPA (InfoNCE) & 520M & 0.58 & 0.60 & 0.55 & 0.66 & 0.58 & 0.55 & 0.59 & 0.25 & 0.07 & 0.12 & 0.18 & 0.06 \\
  IMJEPA & 520M & 0.46 & 0.59 & 0.55 & 0.66 & 0.35 & \underline{0.74} & 0.59 & 0.46 & 0.04 & 0.05 & 0.07 & 0.04 \\
  MLM & 1.15B & 0.41 & 0.55 & 0.55 & 0.65 & 0.27 & 0.73 & 0.59 & 0.39 & 0.04 & 0.04 & 0.06 & 0.04 \\
  Conditioned MLM & 1.15B & 0.41 & 0.55 & 0.53 & 0.66 & 0.27 & 0.73 & 0.53 & 0.41 & 0.04 & 0.04 & 0.05 & 0.04 \\
  Bidirectional TCA & 1.15B & 0.57 & 0.60 & \underline{0.58} & 0.66 & 0.50 & 0.61 & \underline{0.63} & 0.49 & 0.04 & 0.04 & 0.04 & 0.04 \\
  Cross-Modal & 1.15B & \underline{0.61} & 0.60 & 0.49 & 0.66 & 0.52 & 0.48 & 0.42 & 0.43 & 0.04 & 0.05 & 0.05 & 0.05 \\
  Contrastive (CLIP) & 1.15B & 0.43 & 0.60 & 0.50 & 0.66 & 0.40 & 0.70 & 0.47 & 0.50 & 0.04 & 0.07 & 0.06 & 0.06 \\
  Contrastive (DCL) & 1.15B & 0.46 & 0.59 & 0.49 & \textbf{0.69} & 0.47 & 0.64 & 0.39 & \textbf{0.57} & 0.04 & 0.05 & 0.05 & 0.05 \\
  Contrastive (InfoNCE) & 1.15B & 0.45 & 0.60 & 0.51 & 0.66 & 0.39 & 0.69 & 0.46 & \underline{0.52} & 0.05 & 0.09 & 0.06 & 0.05 \\



  \multicolumn{14}{l}{\textbf{[AlphaGenome-ESM2]}} \\
  DPJEPA (CLIP) & 470M & 0.47 & 0.50 & 0.52 & 0.58 & \textbf{0.63} & 0.60 & 0.61 & 0.29 & \textbf{0.36} & \underline{0.31} & \textbf{0.36} & \underline{0.21} \\
  IMJEPA & 470M & 0.47 & 0.46 & 0.50 & 0.56 & 0.33 & 0.30 & 0.57 & 0.20 & 0.06 & 0.09 & 0.21 & 0.13 \\

  \multicolumn{14}{l}{\textbf{[AlphaGenome-E1]}} \\
  DPJEPA (CLIP) & 470M & 0.47 & 0.49 & 0.51 & 0.60 & \textbf{0.63} & 0.60 & \underline{0.63} & 0.32 & 0.32 & \textbf{0.34} & 0.31 & 0.20 \\
  IMJEPA & 470M & 0.46 & 0.46 & 0.49 & 0.55 & 0.28 & 0.26 & 0.53 & 0.19 & 0.08 & 0.15 & 0.22 & 0.12 \\

      \bottomrule
  \end{tabular}
  }
  \end{table*}

==> tables/zero-shot_with_non_coding_LOCO.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Zero-shot variant effect prediction evaluation across metrics. \textbf{Bold}: best in column. \textit{Italic}: second best in column. \underline{Underlined}: best in column among models with parameter count $\leq$ IsoAlign. \textbf{\underline{Bold + underlined}}: highest value across all metrics within a given dataset.}
  \label{tab:zero-shot-eval}

  \resizebox{\textwidth}{!}{
  \begin{tabular}{lccccccccccccccccc}
      \toprule
      & & \multicolumn{4}{c}{ClinVar Missense}
      & \multicolumn{4}{c}{ClinVar Splicing}
      & \multicolumn{4}{c}{ClinVar Non-Coding}
      & \multicolumn{4}{c}{MFASS} \\

      \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14} \cmidrule(l){15-18}

      Model & Params
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul \\

      \midrule

      \multicolumn{18}{l}{\textbf{Baselines}} \\
      AlphaGenome~\citep{avsec2025alphagenome} & 450M & 0.46 & 0.47 & 0.51 & 0.58 & \textit{0.61} & 0.57 & \textit{\underline{0.63}} & 0.30 & 0.71 & 0.69 & 0.65 & \textit{0.44} & 0.29 & \textit{0.31} & \textit{0.32} & \textbf{0.23} \\
      NTv2-500M~\citep{dalla2025nucleotide} & 500M & 0.40 & 0.54 & 0.52 & 0.66 & 0.32 & 0.73 & 0.52 & 0.42 & 0.44 & 0.77 & 0.49 & 0.40 & 0.04 & 0.04 & 0.05 & 0.04 \\
      \midrule
      DNABERT-2~\citep{zhou2023dnabert} & 117M & 0.44 & 0.45 & 0.46 & 0.58 & 0.14 & 0.15 & 0.18 & 0.18 & 0.35 & 0.33 & 0.35 & 0.42 & 0.04 & 0.04 & 0.05 & 0.04 \\
      HyenaDNA \citep{nguyen2023hyenadna} & 1.6M & 0.48 & 0.49 & 0.49 & 0.54 & 0.17 & 0.18 & 0.25 & 0.18 & 0.36 & 0.40 & 0.47 & 0.36 & 0.04 & 0.04 & 0.05 & 0.04 \\
      HyenaDNA-tiny & & 0.46 & 0.46 & 0.49 & 0.53 & 0.16 & 0.15 & 0.22 & 0.17 & 0.37 & 0.38 & 0.44 & 0.36 & 0.04 & 0.04 & 0.04 & 0.04 \\
      Caduceus-PH \citep{schiff2024caduceus} & 7.7M & 0.46 & 0.48 & 0.48 & 0.58 & 0.20 & 0.18 & 0.19 & 0.19 & 0.39 & 0.40 & 0.36 & 0.37 & 0.04 & 0.04 & 0.05 & 0.05 \\
      Caduceus-PS & 7.7M & 0.46 & 0.47 & 0.49 & 0.61 & 0.20 & 0.45 & 0.42 & 0.42 & 0.39 & 0.47 & 0.41 & 0.37 & 0.04 & 0.08 & 0.13 & 0.10 \\
      LucaOne~\citep{he2025generalized} & 1.8B & 0.46 & 0.47 & 0.46 & 0.50 & 0.15 & 0.16 & 0.18 & 0.17 & 0.35 & 0.38 & 0.36 & 0.37 & 0.05 & 0.06 & 0.09 & 0.07 \\
      LucaOne-gene & 1.8B & 0.47 & 0.46 & 0.47 & 0.51 & 0.15 & 0.17 & 0.18 & 0.17 & 0.37 & 0.36 & 0.36 & 0.39 & 0.05 & 0.06 & 0.08 & 0.06 \\
      Orthrus-4track~\citep{fradkin2026orthrus} & 10M & 0.47 & 0.46 & 0.46 & 0.48 & 0.18 & 0.16 & 0.14 & 0.16 & 0.36 & 0.35 & 0.35 & 0.35 & 0.04 & 0.04 & 0.04 & 0.04 \\
      Orthrus-MLM & & 0.49 & 0.53 & 0.46 & 0.59 & 0.18 & 0.19 & 0.15 & 0.19 & 0.38 & 0.39 & 0.35 & 0.37 & 0.04 & 0.04 & 0.04 & 0.04 \\
      Omni-DNA-116M \citep{li2025omni} & 116M & 0.45 & 0.44 & 0.54 & 0.62 & 0.15 & 0.15 & 0.55 & 0.21 & 0.35 & 0.34 & 0.57 & \textbf{0.58} & 0.04 & 0.04 & 0.10 & 0.06 \\
      Omni-DNA-300M & 300M & 0.45 & 0.44 & 0.50 & 0.63 & 0.15 & 0.14 & 0.49 & 0.21 & 0.35 & 0.33 & 0.44 & \textbf{0.58} & 0.04 & 0.04 & 0.13 & 0.06 \\
      AIDO.DNA-300M \citep{ellington2024accurate} & 300M & 0.59 & \underline{0.62} & 0.54 & 0.66 & 0.52 & 0.58 & 0.52 & \textit{0.52} & 0.49 & 0.74 & 0.47 & 0.36 & 0.05 & 0.09 & 0.12 & 0.07 \\
      NTv3-650M \citep{boshar2025foundational} & 650M & 0.56 & 0.50 & 0.48 & 0.66 & 0.35 & 0.57 & 0.34 & 0.28 & 0.38 & 0.63 & 0.37 & 0.37 & 0.04 & 0.07 & 0.08 & 0.07 \\
      NTv3-100M & 100M & 0.50 & 0.55 & 0.46 & 0.62 & 0.51 & 0.66 & 0.22 & 0.21 & 0.55 & 0.67 & 0.37 & 0.37 &  0.10 & 0.12 & 0.07 & 0.08 \\
      Evo2-1B-base~\citep{brixi2026genome} & 1B & 0.56 & \textit{0.77} & 0.57 & \textit{0.67} & 0.38 & \textit{0.85} & 0.59 & 0.35 & 0.58 & \textbf{\underline{0.89}} & 0.48 & 0.39 & 0.05 & 0.16 & 0.16 & 0.10 \\
      Evo2-7B-base & 7B & \textbf{0.70} & \textbf{\underline{0.79}} & \textbf{\underline{0.79}} & \textit{0.67} & 0.57 & \textbf{\underline{0.88}} & \textbf{0.72} & 0.36 & 0.67 & \textbf{\underline{0.89}} & \textbf{0.70} & 0.42 & 0.05 & 0.09 & 0.13 & 0.13 \\
      Carbon & 3B & 0.79 & 0.83 & 0.79 & 0.81 & 0.63 & 0.90 & 0.65 & 0.75 & 0.59 & 0.87 & 0.55 & 0.42 & 0.05 & 0.08 & 0.09 & 0.06 \\
      JEPA-NTv3-100M & & 0.62 & 0.52 & 0.46 & 0.62 & 0.47 & 0.55 & 0.25 & 0.20 & 0.55 & 0.59 & 0.37 & 0.36 & 0.12 & 0.08 & 0.08 & 0.08 \\
      JEPA-DNABERT-2 & & 0.45 & 0.44 & 0.49 & 0.57 & 0.14 & 0.15 & 0.27 & 0.19 & 0.33 & 0.33 & 0.37 & 0.45 & 0.04 & 0.04 & 0.08 & 0.04 \\
      JEPA-HyenaDNA-tiny & & 0.45 & 0.46 & 0.47 & 0.51 & 0.15 & 0.16 & 0.19 & 0.17 & 0.34 & 0.33 & 0.40 & 0.36 & 0.04 & 0.04 & 0.04 & 0.03 \\
      
      
      
      
      \midrule
      \multicolumn{18}{l}{\textbf{IsoAlign}} \\
      \midrule
      \multicolumn{18}{l}{\textbf{ NT} [ESM2]} \\
      DP-JEPA (CLIP) & 520M & 0.55 & 0.61 & 0.54 & \textit{0.67} & \textbf{0.63} & 0.67 & 0.47 & 0.46 & 0.68 & \textit{\underline{0.79}} & 0.46 & 0.35 & 0.08 & 0.17 & 0.18 & 0.08 \\
      DP-JEPA (DCL) & 520M & 0.58 & \underline{0.62} & 0.55 & 0.65 & 0.39 & 0.47 & 0.49 & 0.24 & 0.51 & 0.61 & 0.44 & 0.34 & 0.05 & 0.06 & 0.10 & 0.06 \\
      DP-JEPA (InfoNCE) & 520M & 0.58 & 0.60 & 0.55 & 0.66 & 0.58 & 0.55 & 0.59 & 0.25 & 0.52 & 0.61 & 0.51 & 0.34 & 0.07 & 0.12 & 0.18 & 0.06 \\
      IM-JEPA & 520M & 0.46 & 0.59 & 0.55 & 0.66 & 0.35 & \underline{0.74} & 0.59 & 0.46 & 0.47 & \textit{\underline{0.79}} & 0.57 & 0.33 & 0.04 & 0.05 & 0.07 & 0.04 \\
      MLM & 520M & 0.41 & 0.55 & 0.55 & 0.65 & 0.27 & 0.73 & 0.59 & 0.39 & 0.43 & 0.75 & 0.52 & 0.33 & 0.04 & 0.04 & 0.06 & 0.04 \\
      Conditioned MLM & 520M & 0.41 & 0.55 & 0.53 & 0.66 & 0.27 & 0.73 & 0.53 & 0.41 & 0.46 & 0.78 & 0.48 & 0.38 & 0.04 & 0.04 & 0.05 & 0.04 \\
      Bidirectional TCA & 520M & 0.57 & 0.60 & \textit{\underline{0.58}} & 0.66 & 0.50 & 0.61 & \textit{\underline{0.63}} & 0.49 & 0.43 & 0.59 & 0.55 & 0.35 & 0.04 & 0.04 & 0.04 & 0.04 \\
      Cross-Modal & 520M & \textit{\underline{0.61}} & 0.60 & 0.49 & 0.66 & 0.52 & 0.48 & 0.42 & 0.43 & 0.46 & 0.58 & 0.42 & 0.40 & 0.04 & 0.05 & 0.05 & 0.05 \\
      Contrastive (CLIP) & 520M & 0.43 & 0.60 & 0.50 & 0.66 & 0.40 & 0.70 & 0.47 & 0.50 & 0.46 & 0.76 & 0.47 & 0.35 & 0.04 & 0.07 & 0.06 & 0.06 \\
      Contrastive (DCL) & 520M & 0.46 & 0.59 & 0.49 & \textbf{0.69} & 0.47 & 0.64 & 0.39 & \textbf{0.57} & 0.51 & 0.74 & 0.44 & 0.40 & 0.04 & 0.05 & 0.05 & 0.05 \\
      Contrastive (InfoNCE) & 520M & 0.45 & 0.60 & 0.51 & 0.66 & 0.39 & 0.69 & 0.46 & \textit{0.52} & 0.46 & 0.76 & 0.46 & 0.37 & 0.05 & 0.09 & 0.06 & 0.05 \\

      \multicolumn{18}{l}{\textbf{ AlphaGenome} [ESM2]}\\
      DP-JEPA (CLIP) & 470M & 0.47 & 0.50 & 0.52 & 0.58 & \textbf{0.63} & 0.60 & 0.61 & 0.29 & \textbf{0.74} & 0.76 & \textit{\underline{0.68}} & \textit{0.44} & \textbf{\underline{0.36}} & \textit{0.31} & \textbf{\underline{0.36}} & \textit{0.21} \\
      IM-JEPA & 470M & 0.47 & 0.46 & 0.50 & 0.56 & 0.33 & 0.30 & 0.57 & 0.20 & 0.46 & 0.45 & 0.49 & 0.35 & 0.06 & 0.09 & 0.21 & 0.13 \\

      \multicolumn{18}{l}{\textbf{ AlphaGenome} [E1]} \\
      DP-JEPA (CLIP) & 470M & 0.47 & 0.49 & 0.51 & 0.60 & \textbf{0.63} & 0.60 & \textit{\underline{0.63}} & 0.32 & \textit{0.72} & 0.71 & 0.63 & 0.41 & \textit{0.32} & \textbf{0.34} & 0.31 & 0.20 \\
      IM-JEPA & 470M & 0.46 & 0.46 & 0.49 & 0.55 & 0.28 & 0.26 & 0.53 & 0.19 & 0.44 & 0.43 & 0.46 & 0.35 & 0.08 & 0.15 & 0.22 & 0.12 \\

      \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/zero-shot_with_splicing.tex <==
\begin{table*}[htbp]                           
  \centering
  \caption{Zero-shot variant effect prediction evaluation across metrics}
  \label{tab:zero-shot-eval}              

  \resizebox{\textwidth}{!}{                                                                                                                                                                                  
  \begin{tabular}{lccccccccccccc}
      \toprule                                                                                                                                                                                                
      & & \multicolumn{4}{c}{ClinVar missense}                                                                                                                                                              
      & \multicolumn{4}{c}{ClinVar Splicing}
      & \multicolumn{4}{c}{MFASS} \\

      \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14}

      Model & Params
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul
      & Cos & L2 & CLS & Mul \\

      \midrule

      \multicolumn{14}{l}{\textbf{Baselines}} \\
  AlphaGenome & 450M & 0.46 & 0.47 & 0.51 & 0.71 & - & - & - & - & 0.29 & 0.31 & 0.42 & 0.58 \\
  NTv2 & 500M & 0.40 & 0.54 & 0.51 & 0.69 & 0.66 & 0.70 & 0.47 & 0.61 & 0.04 & 0.04 & 0.05 & 0.11 \\
  DNABERT-2 & 117M & 0.44 & 0.45 & 0.47 & 0.66 & - & - & - & - & 0.04 & 0.04 & 0.05 & 0.09 \\
  HyenaDNA & 1.6M & 0.48 & 0.49 & 0.49 & 0.60 & - & - & - & - & 0.04 & 0.04 & 0.05 & 0.08 \\
  Caduceus-PH & 7.7M & 0.46 & 0.48 & 0.48 & 0.64 & - & - & - & - & 0.04 & 0.04 & 0.04 & 0.10 \\
  Caduceus-PS & 7.7M & 0.46 & 0.47 & 0.50 & 0.66 & - & - & - & - & 0.04 & 0.08 & 0.14 & 0.17 \\
  LucaOne & 1.8B & 0.46 & 0.47 & 0.46 & 0.61 & - & - & - & - & 0.05 & 0.06 & 0.11 & 0.22 \\
  LucaOne-gene & 1.8B & 0.47 & 0.46 & 0.46 & 0.61 & - & - & - & - & 0.05 & 0.06 & 0.09 & 0.23 \\
  Omni-DNA-116M & 116M & 0.45 & 0.44 & 0.54 & 0.69 & - & - & - & - & 0.04 & 0.04 & 0.10 & 0.13 \\
  Omni-DNA-300M & 300M & 0.45 & 0.44 & 0.50 & 0.70 & - & - & - & - & 0.04 & 0.04 & 0.16 & 0.14 \\
  AIDO.DNA-300M & 300M & 0.59 & 0.62 & 0.54 & 0.73 & - & - & - & - & 0.05 & 0.09 & 0.13 & 0.24 \\
  NTv3-650M & 650M & 0.56 & 0.50 & 0.48 & 0.76 & - & - & - & - & 0.04 & 0.07 & 0.13 & 0.27 \\
  Evo2-7B-base & 7B & \textbf{0.70} & \textbf{0.79} & \textbf{0.77} & \textbf{0.78} & - & - & - & - & 0.05 & 0.09 & 0.24 & 0.43 \\

      \midrule

      \multicolumn{14}{l}{\textbf{Ours [NT-ESM2]}} \\
      DPJEPA (CLIP) & 520M & \textbf{0.62} & \textbf{0.68} & 0.52 & \textbf{0.75} & 0.66 & 0.70 & 0.46 & 0.61 & 0.05 & 0.07 & 0.08 & 0.12 \\
      IMJEPA & 520M & 0.53 & 0.64 & 0.54 & 0.72 & 0.37 & 0.71 & 0.61 & 0.56 & 0.04 & 0.04 & 0.06 & 0.12 \\
      Bidirectional TCA & 1.15B & 0.57 & 0.60 & \textbf{0.57} & 0.72 & 0.58 & 0.68 & \textbf{0.69} & 0.61 & 0.04 & 0.04 & 0.05 & 0.11 \\
      DPJEPA (InfoNCE) & 520M & 0.58 & 0.60 & 0.55 & 0.72 & 0.66 & 0.61 & 0.65 & 0.37 & 0.07 & 0.12 & 0.15 & 0.22 \\
      MLM & 1.15B & 0.41 & 0.55 & 0.54 & 0.69 & 0.35 & 0.77 & 0.65 & 0.53 & 0.04 & 0.04 & 0.07 & 0.10 \\
      Conditioned MLM & 1.15B & 0.41 & 0.57 & 0.52 & 0.70 & 0.32 & \textbf{0.78} & 0.60 & 0.53 & 0.04 & 0.04 & 0.05 & 0.10 \\
      DPJEPA (DCL) & 520M & 0.58 & 0.62 & 0.54 & 0.72 & 0.51 & 0.56 & 0.55 & 0.37 & 0.05 & 0.06 & 0.11 & 0.14 \\
      Contrastive (CLIP) & 1.15B & 0.43 & 0.60 & 0.50 & 0.71 & 0.48 & 0.76 & 0.55 & 0.64 & 0.04 & 0.07 & 0.07 & 0.12 \\
      Contrastive (InfoNCE) & 1.15B & 0.45 & 0.60 & 0.50 & 0.71 & 0.47 & 0.75 & 0.54 & 0.64 & 0.05 & 0.09 & 0.07 & 0.13 \\
      Cross-Modal & 1.15B & 0.61 & 0.60 & 0.50 & 0.72 & 0.59 & 0.57 & 0.49 & 0.54 & 0.04 & 0.05 & 0.06 & 0.09 \\
      Contrastive (DCL) & 1.15B & 0.46 & 0.59 & 0.49 & 0.74 & 0.54 & 0.71 & 0.45 & \textbf{0.70} & 0.04 & 0.05 & 0.05 & 0.12 \\

      \multicolumn{14}{l}{\textbf{[AlphaGenome-ESM2]}} \\
      AlphaGenome-ESM2 & 470M & 0.46 & 0.48 & 0.51 & 0.71 & \textbf{0.69} & 0.67 & 0.66 & 0.49 & 0.33 & 0.27 & 0.40 & \textbf{0.59} \\

      \multicolumn{14}{l}{\textbf{[AlphaGenome-E1]}} \\
      AlphaGenome-E1 & 470M & 0.46 & 0.48 & 0.51 & 0.72 & 0.69 & 0.66 & 0.67 & 0.49 & \textbf{0.37} & \textbf{0.35} & \textbf{0.41} & 0.57 \\

      \bottomrule
  \end{tabular}
  }
  \end{table*}
